Generalized and Incremental Few-Shot Learning by Explicit Learning and Calibration without Forgetting

Both generalized and incremental few-shot learning have to deal with three major challenges: learning novel classes from only few samples per class, preventing catastrophic forgetting of base classes, and classifier calibration across novel and base classes. In this work we propose a three-stage framework that allows to explicitly and effectively address these challenges. While the first phase learns base classes with many samples, the second phase learns a calibrated classifier for novel classes from few samples while also preventing catastrophic forgetting. In the final phase, calibration is achieved across all classes. We evaluate the proposed framework on four challenging benchmark datasets for image and video few-shot classification and obtain state-of-the-art results for both generalized and incremental few shot learning.

==> b_b_backbones.tex <==
%!TEX root = ../main.tex


\begin{table}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{ccc}  % 4 = method, model, gn(5/69), gb(64/69), hm
\toprule
GFSL && \\
% \multicolumn{7}{c}{mini-ImageNet} \\
% & \multicolumn{3}{c}{5w1s}  \\
% & & $\text{N}_{/J}$  & $\text{B}_{/J}$  & $\text{hm}_{/J}$ \\
% &  (5/69) & (64/69) &  \\
\midrule
CONV4~\cite{shi2019relational} & \multirow{2}{*}{mini} & 70.08 \\
CONV4 (ours) & & 73.02 \\
\midrule
ResNet10~\cite{gidaris2018dynamic}  & \multirow{3}{*}{mini}  & 70.15 \\
ResNet10~\cite{ren2019incremental} (modified) &  & 77.64 \\
ResNet12 (ours) &  & 79.94 \\
\midrule
ResNet18~\cite{ren2019incremental}  & \multirow{2}{*}{tiered}  & 62.26 \\
ResNet12 (ours) &  & 70.62 \\
\midrule
IFSL && \\
\midrule
ResNet18~\cite{chen2021incremental}  & \multirow{2}{*}{mini}  & - \\
ResNet18 (ours) &  & - \\
\bottomrule
\end{tabular}

\caption{$B_{/B}$ performance after the first phase on the base classes with the pretrained backbone on the base classes for (our) and after the method for others.}
\label{table:b_b_backbones}
\vspace{-5mm}
\end{table}

==> replay_sampling.tex <==
%!TEX root = ../main.tex

\begin{table}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|ccc|ccc}  % 7 = method, model, gn(5/69), gb(64/69), hm
\toprule
% \multicolumn{7}{c}{mini-ImageNet} \\
& \multicolumn{3}{c|}{5w1s} & \multicolumn{3}{c}{5w5s} \\
% \multirow{2}{*}{method}  & $\text{N}^{\uplus}$  & $\text{B}^{\uplus}$  & \multirow{2}{*}{$\text{hm}^{\uplus}$} & $\text{N}^{\uplus}$ & $\text{B}^{\uplus}$  & \multirow{2}{*}{$\text{hm}^{\uplus}$} \\
sampling & $\text{N}^{\uplus}$  & $\text{B}^{\uplus}$  & \multirow{2}{*}{$\text{hm}^{\uplus}$} & $\text{N}^{\uplus}$ & $\text{B}^{\uplus}$  & \multirow{2}{*}{$\text{hm}^{\uplus}$} \\
method & (5/69) & (64/69) &  & (5/69) & (64/69) &  \\
\midrule
fixed & 53.28 & 63.24 & 57.83 & 68.61 & 64.73 & 66.61 \\
random & 53.50 & 63.56 & 58.10 & 67.65 & 66.57 & 67.10 \\

\bottomrule
\end{tabular}

\caption{Replay sampling during 3rd phase, mini-ImageNet, 100 episodes}
\label{table:replay_sampling}
\end{table}

==> sota_incremental_old.tex <==
%!TEX root = ../main.tex

\begin{table*}[!t]
\centering
\footnotesize
\tabcolsep=0.15cm
\begin{tabular}{c|cccccccc}  % 10 = method, 1,.. 9 
\toprule
\multicolumn{9}{c}{mini-ImageNet} \\
method  & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
$hm_{/J}$ & $+5$ & $+10$ & $+15$ & $+20$ & $+25$ & $+30$ & $+35$ & $+40$  \\
\midrule
FT$^\diamond$ & 7.23 & 7.39 & 4.87 & 2.40 & 2.06 & 1.84 & 1.57 & 1.40  \\
Joint$^\diamond$ & 8.92 & 17.02 & 21.86 & 20.54 & 22.92 & 22.85 & 24.41 & 24.95  \\
\midrule
iCaRL~\cite{rebuffi2017icarl}$^\diamond$  & 8.45 & 13.86 & 14.92 & 13.00 & 14.06 & 12.74 & 12.16 & 11.71  \\
UCIR~\cite{hou2019learning}$^\diamond$ & 9.62 & 14.14 & 15.58 & 13.19 & 13.63 & 13.11 & 12.76 & 11.96  \\
PN~\cite{snell2017prototypical}$^\diamond$ & 9.76 & 14.72 & 16.78 & 19.09 & 20.06 & 19.37 & 18.98 & 18.90  \\
ILVQ~\cite{xu2012ilvq}$^\diamond$ & 9.66 & 16.08 & 17.78 & 20.05 & 20.35 & 19.64 & 19.06 & 18.89  \\
SDC~\cite{yu2020sdc}$^\diamond$  & 20.51 & 18.79 & 17.36 & 20.47 & 19.21 & 18.27 & 20.79 & 21.77  \\
IW~\cite{qi2018imprinted}$^\diamond$  & 25.32 & 20.45 & 22.62 & 25.48 & 22.54 & 20.66 & 21.27 & 22.27  \\
IDLVQ~\cite{chen2021incremental} & 21.69 & 20.44 & 21.98 & 25.19 & 22.99 & 20.82 & 21.56 & 22.65  \\
\midrule
% BLF (base biased) & 25.56 & 30.59 & 27.29 & 28.08 & 29.91 & 27.97 & 30.30 & 32.73  \\
BLF & \textbf{41.24} & \textbf{38.96} & \textbf{39.08} & \textbf{38.67} & \textbf{36.75} & \textbf{35.47} & \textbf{34.71} & \textbf{35.02}  \\

\bottomrule
\end{tabular}

\caption{\bernt{please provide a sensible caption - we are very close to the deadline} sota incremental few-shot learning hm}
\label{table:incremental_sota_hm}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!t]
\centering
\footnotesize
\tabcolsep=0.15cm
\begin{tabular}{c|ccccccccc}  % 10 = method, 1,.. 9 
\toprule
\multicolumn{10}{c}{mini-ImageNet}  \\
$B_{/J}$ ($60$) & 2 &  5 &  7  & 9 \\
\midrule
% FT$^\diamond$  & 32.28 & 3.17 & 1.92 & 1.46  \\
Joint$^\diamond$  & 63.30 &  62.18 & 61.86  & 61.89  \\

SDC~\cite{yu2020sdc}$^\diamond$ & 63.58  & 60.29  & 59.05  & 59.87  \\
IW~\cite{qi2018imprinted}$^\diamond$ & 63.52 & 61.17  & 60.63  & 59.64  \\
IDLVQ~\cite{chen2021incremental} & 63.77  & 61.22  & 60.97 & 60.44  \\
\midrule
BLF (balanced hm)  & 57.33 & 51.38  & 47.60 & 47.73  \\

\midrule
\midrule
% \multicolumn{10}{c}{mini-ImageNet}  \\
$\text{N}^{\uplus}$ & 2 &  5  & 7  & 9 \\
$\#cl$& - & $5$ & $10$ & $15$ & $20$ & $25$ & $30$ & $35$ & $40$  \\
\midrule
% FT$^\diamond$ & 4.07 &  1.93 & 1.77 & 1.36  \\
Joint$^\diamond$ & 4.80 & 12.30 & 14.01 & 15.62  \\

SDC~\cite{yu2020sdc}$^\diamond$  & 12.23 &  12.33  & 10.81  & 13.69  \\
IW~\cite{qi2018imprinted}$^\diamond$  & 15.81 &  16.09 & 12.45 & 13.69  \\
IDLVQ~\cite{chen2021incremental}  & 13.07 & 15.86  & 12.55  & 13.94  \\
\midrule
BLF (balanced hm) & \textbf{32.20} & \textbf{31.12}  & \textbf{28.27} & \textbf{27.65}  \\

\bottomrule
\end{tabular}

\caption{Incremental few shot learning. Joint accuracy on base ($60$ classes) and novel ($X$) classes separately.}
\label{table:incremental_sota_b_and_n}
\end{table*}



==> sota_kinetics_sup_old.tex <==
%!TEX root = ../main.tex

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{Kinetics 5w1s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & N & B & $\text{both}^{\uplus}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (64/64) & (69/69) & (5/69) & (64/69) &  &  \\
 \midrule
 
 PN~\cite{snell2017prototypical} & \multirow{6}{*}{MLP$^*$} & - & - & - & - & - & - & - \\
 IW+FT~\cite{qi2018imprinted} &  & 62.57 & 58.42 & - & 45.56 & 48.56 & 47.01 & 47.06 \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & 65.35 & 56.04 & 47.66 & 50.81 & 44.51 & 47.45 & 47.66 \\
 GFSVC~\cite{xian2020generalized} &  & - & - & 83.26 & 13.70 & 88.70 & 23.73 & 51.20 \\
 IFSwAAN~\cite{ren2019incremental}(code) &  & 59.36 & 57.99 & - & 46.13 & 35.96 & 40.41 & 41.01 \\ 
 BLF (ours) fix sampl &  & 55.97 & 64.84 & - & 47.51 & 50.84 & 49.12 & 49.18 \\
 BLF (ours) rand sampl &  & - & - & - & - & - & - & - \\
%  BLF (ours) & fix & 56.71 & 64.75 & - & 48.18 & 50.82 & 49.46 & 49.50 \\

\bottomrule
\end{tabular}

\caption{\bernt{please provide a sensible caption - we are very close to the deadline} sota Kinetics 5w1s}
\label{table:kinetics_sota_5w1s}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{Kinetics 5w5s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & N & B & $\text{both}^{\uplus}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (64/64) & (69/69) & (5/69) & (64/69) &  &  \\
 \midrule

 PN~\cite{snell2017prototypical} & \multirow{6}{*}{MLP$^*$} & - & - & - & - & - & - & - \\
 IW+FT~\cite{qi2018imprinted} &   & 74.61 & 56.67 & - & 56.92 & 49.17 & 52.76 & 53.04 \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & 81.11 & 56.46 & 58.30 & 70.29 & 46.31 & 55.83 & 58.30 \\
 GFSVC~\cite{xian2020generalized} &  & - & - & - & 22.30 & 88.70 & 35.64 & 55.50 \\
 IFSwAAN~\cite{ren2019incremental} (code) &  & 76.83 & 59.48 & - & 56.99 & 43.21 & 49.15 & 50.10 \\ 
 BLF (ours) fix sampl &  & 74.76 & 65.06 & - & 63.65 & 54.55 & 58.75 & 59.10 \\
 BLF (ours) rand sampl &  & - & - & - & - & - & - & - \\
%  BLF (ours) & fix & 74.35& 65.85 & - & 64.10 & 54.54 & 58.93 & 59.32 \\

\bottomrule
\end{tabular}

\caption{sota Kinetics 5w5s}
\label{table:kinetics_sota_5w5s}
\end{table*}

==> sota_mini_sup.tex <==
%!TEX root = ../main.tex

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{mini-ImageNet 5w1s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & $N_{/J}$ & B & $J_{/J}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (64/64) & (69/69) & (5/69) & (64/69) &  &  \\
 \midrule
 PN~\cite{snell2017prototypical} & \multirow{6}{*}{4CONV} & 53.88 & 54.02 & ? & 0.02 & 54.02 & 0.04 & 27.02 \\
 IW+FT~\cite{qi2018imprinted} &  & - & - & - & - & - & - & - \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & 55.80 & 69.93 & ? & 40.30 & 58.54 & 47.74 & 49.42 \\
 RGFSL~\cite{shi2019relational} &  & 55.08 & 65.14 & ? & 39.86 & 54.65 & 46.10 & 47.25 \\ 
 RGFSL~\cite{shi2019relational} + WordNet &  & 60.40 & 68.13 & ? & 48.59 & 54.68 & 51.45 & 51.63 \\ 
 LCwoF (ours) &  & 58.32 & 72.75 & 54.50 & 47.16 & 55.07 & 50.81 & 51.12 \\
 
 \midrule
 
  PN~\cite{snell2017prototypical} & \multirow{7}{*}{ResNet} & - & - & - & - & - & - & 42.73~\cite{ren2019incremental} \\
   IW+FT~\cite{qi2018imprinted}(reimpl) &  & 47.17 & 61.78 & - & 31.25 & 47.72 & 37.77 & 39.49 \\
%  IW+FT~\cite{qi2018imprinted} &  & 67.56 & 69.07 & - & 46.96 & 58.92 & 52.26 & 52.94 \\
 DFSLwoF~\cite{gidaris2018dynamic} (code) &  & 56.83 & 70.15 & 49.68 (51.23) & 41.32 & 58.04 & 48.27 & 49.68 \\
%  DAE-GNN~\cite{gidaris2019generating} (WRN) &  & 61.07 & - & 56.55~\cite{gidaris2019generating} & - & - & - & - \\ 51.23
 IFSwAAN~\cite{ren2019incremental}(code) &  & 56.14 & 77.58 & 62.59(?) & 45.61 & 63.92 & 53.24 & 54.76 (54.95) \\ 
 LCwoF (ours) fix sampl &  & 60.78 & 79.89 & 62.15 & 52.78 & 62.89 & 57.39 & 57.84 \\
 LCwoF (ours) rand sampl &  & 61.15 & 80.10 & - & 53.33 & 62.99 & 57.75 & 58.16 \\
%   \midrule
%  BLF (ours) fix sampl & fix & 60.97 & 79.89 & - & 52.95 & 63.08 & 57.57 & 58.02 \\
%  BLF (ours) rand sampl & fix & 61.20 & 80.08 & - & 53.42 & 63.12 & 57.87 & 58.27 \\
\bottomrule
\end{tabular}

\caption{\bernt{please provide a sensible caption - we are very close to the deadline} sota mini-ImageNet 5w1s}
\label{table:mini_sota_5w1s}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{mini-ImageNet 5w5s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & N & B & $J_{/J}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (64/64) & (69/69) & (5/69) & (64/69) &  &  \\
 \midrule
 PN~\cite{snell2017prototypical} & \multirow{6}{*}{4CONV} & 70.84 & 60.42 & ? & 2.99 & 60.41 & 5.70 & 31.70 \\
 IW~\cite{qi2018imprinted} &  & - & - & - & - & - & - & - \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & 72.24 & 70.24 & ? & 58.26 & 59.89 & 59.06 & 59.07 \\
 RGFSL~\cite{shi2019relational} &  & 72.32 & 67.79 & ? & 56.32 & 59.30 & 57.71 & 57.81 \\ 
 RGFSL~\cite{shi2019relational} + WordNet &  & 73.31 & 68.30 & ? & 59.32 & 57.93 & 58.62 & 58.63 \\ 
 BLF (ours) &  & 73.63 & 71.82 & 60.10 & 62.23 & 59.94 & 61.06 & 61.09 \\
 
 \midrule
 
  PN~\cite{snell2017prototypical} & \multirow{7}{*}{ResNet} & - & - & - & - & - & - & 57.05 \\
 IW+FT~\cite{qi2018imprinted}(reimpl) &  & 67.56 & 69.07 & - & 46.96 & 58.92 & 52.26 & 52.94 \\
 DFSLwoF~\cite{gidaris2018dynamic} (code) &  & 72.82 & 70.03 & 58.98 & 59.27 & 58.68 & 58.97 & 58.98 \\
%  DAE-GNN~\cite{gidaris2019generating} (WRN) &  & 76.75 & - & 67.00 & - & - & - & - \\
 IFSwAAN~\cite{ren2019incremental} (code) &  & 69.72 & 77.58 & 63.89(?) & 60.82 & 64.14 & 62.43 & 62.48 (63.04) \\ 
 BLF (ours) fix sampl &  & 77.65 & 79.96 & 64.74 & 68.58 & 64.53 & 66.49 & 66.55 \\
 BLF (ours) rand sampl &  & 77.88 & 80.09 & - & 67.17 & 66.59 & 66.88 & 66.88 \\
%   \midrule
%  BLF (ours) fix sampl & fix  & 76.45 & 79.86 & - & 70.27 & 63.14 & 66.51 & 66.71 \\
%  BLF (ours) rand sampl & fix  & 76.77 & 80.07 & - & 69.46 & 65.21 & 67.27 & 67.34 \\

 
\bottomrule

\end{tabular}

\caption{sota mini-ImageNet 5w5s}
\label{table:mini_sota_5w5s}
\end{table*}

==> sota_tiered_sup_old.tex <==
%!TEX root = ../main.tex

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{tiered-ImageNet 5w1s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & N & B & $\text{both}^{\uplus}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (200/200) & (205/205) & (5/205) & (200/205) &  &  \\
 \midrule
 
 PN~\cite{snell2017prototypical} & \multirow{5}{*}{ResNet} & - & - & - & - & - & - & 30.04 \\
 IW+FT~\cite{qi2018imprinted} &  & 60.88 & 70.19 & - & 44.95 & 62.53 & 52.30 & 52.74 \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & - & - & - & - & - & - & 52.40 \\
 IFSwAAN~\cite{ren2019incremental} &  & 61.37 & 62.44 & 55.81(?) & 54.39 & 55.85 & 55.11 & 55.12 (56.11) \\ 
%  BLF (ours) fixed &  & 65.37 & 70.55 & 60.37 & 57.85 & 60.44 & 59.12 & 59.15 \\
 BLF (ours) fix sampl &  & 64.71 & 70.55 & 60.31 & 57.13 & 60.39 & 58.71 & 58.76 \\
 BLF (ours) rand sampl &  & 64.67 & 70.59 & - & 59.79 & 60.86 & 58.75 & 58.82 \\
%   \midrule
%  BLF (ours) fix sampl & fix  & 65.33 & 70.54 & - & 57.33 & 61.22 & 59.21 & 59.28 \\
%  BLF (ours) rand sampl & fix  & 65.67 & 70.59 & - & 58.60 & 60.24 & 59.41 & 59.42 \\
 

\bottomrule
\end{tabular}

\caption{\bernt{please provide a sensible caption - we are very close to the deadline} sota tiered-ImageNet 5w1s}
\label{table:tiered_sota_5w1s}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[!t]
\centering
\small
\tabcolsep=0.15cm
\begin{tabular}{c|c|cc|c|cc|cc}  % 9 = method, model, n (5/5), b (64/64), both (69/69), gn(5/69), gb(64/69), hm, am
\toprule
\multicolumn{9}{c}{tiered-ImageNet 5w5s} \\
\multirow{2}{*}{method} & \multirow{2}{*}{model} & N & B & $\text{both}^{\uplus}$ & $N_{/J}$  & $B_{/J}$  & \multirow{2}{*}{$hm_{/J}$} & \multirow{2}{*}{$\text{am}^{\uplus}$} \\
 &  & (5/5) & (200/200) & (205/205) & (5/205) & (200/205) &  &  \\
 \midrule
 
 PN~\cite{snell2017prototypical} & \multirow{5}{*}{ResNet} & - & - & - & - & - & - & 41.38 \\
 IW+FT~\cite{qi2018imprinted} &  & 79.26 & 70.25 & - & 71.85 & 56.11 & 63.01 & 63.98 \\
 DFSLwoF~\cite{gidaris2018dynamic} &  & - & - & - & - & - & - & 62.63 \\
 IFSwAAN~\cite{ren2019incremental} &  & 77.91 & 62.36 & 58.10(?) & 72.09 & 57.76 & 64.13 & 64.93 (65.52) \\ 
%  BLF (ours) &  & 79.70 & 70.55 & 61.21 & 69.68 & 61.00 & 65.05 & 65.34 \\ % lambda = 1e+4
 BLF (ours) fix sampl &  & 79.72 & 70.58 & 63.58 & 69.05 & 63.44 & 66.12 & 66.25 \\
 BLF (ours) rand sampl &  & 79.67 & 70.59 & - & 70.20 & 63.01 & 66.41 & 66.61 \\
%  \midrule
%  BLF (ours) fix sampl & fix  & - & - & - & - & - & - & - \\
%  BLF (ours) rand sampl & fix  & - & - & - & - & - & - & - \\
 

\bottomrule
\end{tabular}

\caption{sota tiered-ImageNet 5w5s}
\label{table:tiered_sota_5w5s}
\end{table*}
